Scattering Amplitude Techniques in Classical Gauge Theories and Gravity

In this thesis we present a study of the computation of classical observables in gauge theories and gravity directly from scattering amplitudes. In particular, we discuss the direct application of modern amplitude techniques in the one, and two-body problems for both, scattering and bounded scenarios, and in both, classical electrodynamics and gravity, with particular emphasis on spin effects in general, and in four spacetime dimensions. Among these observables we have the conservative linear impulse and the radiated waveform in the two-body problem, and the differential cross section for the scattering of waves off classical spinning compact objects. Implications of classical soft theorems in the computation of classical radiation are also discussed. Furthermore, formal aspects of the double copy for massive spinning matter, and its application in a classical two-body context are considered. Finally, the relation between the minimal coupling gravitational Compton amplitude and the scattering of gravitational waves off the Kerr black hole is presented.

==> preface.tex <==
\chapter*{\centering Preface}
As a final project for the postgraduate diploma programme in High Energy, Cosmology and Astroparticle Physics, of the Abdus Salam
International Center for Theoretical Physics ICTP, I have decided to write this final report. It contains  a basic introduction to 
the very well known $AdS/CFT$ correspondence, proposed by Maldacena \cite{Maldacena}. The topic of the project was suggested by
professor Atish Dabholcar, who also supervised the work.\\
The correspondence states that \textit{a theory of gravity in
$AdS$ background is dynamically equivalent to a Conformal Field Theory (CFT) living in the conformal boundary}. The main aim of this 
work is to understand what this sentence means, and in order to do so, I have divide this text in four chapters. 
In the  first one I did a study of the $AdS_{d+1}$ geometry, trying to understand  the most common  chose of coordinate to parametrize it,
and using
as  main reference  \cite{podolsky}. Having understood this geometry, I ventured to study the basis of Conformal Field Theories, which I 
summarized in the second chapter, for this part, I followed \cite{francesco}. It had came the time to made the link between a theory of 
gravity in $AdS_{d+1}$ spaces and  the dual associated CFT that lives in the boundary. But how to do it without having too much background in
string theory? The answer to this question was: by studying reviews in the topic that do not require it. For this reason I followed 
the Witten\textquotesingle s paper \cite{Witten:1998qj} and other good reviews as \cite{McGreevy:2009xe} and \cite{Aharony}; this last 
one has a very good explanation of the whole topic of the present work.\\ So far all what is contained in these three chapters is just formal, and 
there is not explicit example of which CFT, and the list of operator of it. For this reason I include one last chapter with the 
most commune correspondence which was the one Maldacena proposed between a theory of gravity living in $AdS_4\times S^5$ and 
a Super Yang-Mills theory which is known to be a conformal theory, living in a four dimensional Minkowski space-time. For this last part, I 
followed the original Maldacena\textquotesingle s paper \cite{Maldacena}, and the introductory book to the Gauge-gravity 
duality \cite{johana}.  This last section only include relevant results, without formal derivation, this due to the lake of knowledge
of strong basis in String theory. I hope in the near future I can  fill this hole. Here I just present the most relevant bibliography for 
the work.  Additional bibliography is included along the text.\\
The inclusion of this section in the text is to give some flavor of the organization of the report, since, due to the reduced time to 
do the project, it was not possible to consult many references to include a chapter of introduction, in which it is explained the state of
the art of the topic. \\\\
\rightline{Yilber Fabian Bautista}\\
\rightline{The Abdus Salam ICTP}\\
\rightline{Trieste, Italy}\\
\rightline{2016} 
